SelfEval: Leveraging the discriminative nature of generative models for evaluation

We present an automated way to evaluate the text alignment of text-to-image generative diffusion models using standard image-text recognition datasets. Our method, called SelfEval, uses the generative model to compute the likelihood of real images given text prompts, and the likelihood can be used to perform recognition tasks with the generative model. We evaluate generative models on standard datasets created for multimodal text-image discriminative learning and assess fine-grained aspects of their performance: attribute binding, color recognition, counting, shape recognition, spatial understanding. Existing automated metrics rely on an external pretrained model like CLIP (VLMs) or LLMs, and are sensitive to the exact pretrained model and its limitations. SelfEval sidesteps these issues, and to the best of our knowledge, is the first automated metric to show a high degree of agreement for measuring text-faithfulness with the gold-standard human evaluations across multiple generative models, benchmarks and evaluation metrics. SelfEval also reveals that generative models showcase competitive recognition performance on challenging tasks such as Winoground image-score compared to discriminative models. We hope SelfEval enables easy and reliable automated evaluation for diffusion models.

==> Makefile <==
main:
	pdflatex main

full:
	pdflatex main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main

camready: full
	gs -dNOPAUSE -dBATCH -dNOPLATFONTS -sDEVICE=pdfwrite -dEmbedAllFonts=true -sOutputFile=main-gs.pdf -f main.pdf

cut: full
	pdftk main.pdf cat 1-16 output main_submit.pdf
	pdftk main.pdf cat 17-end 14-16 output suppl_submit.pdf

clean:
	rm *.aux *.bbl *.blg *.log *.pdf *.dep *.brf *.fls *.out

run:
	evince main.pdf

compress:
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/default -dNOPAUSE -dQUIET -dBATCH -dDetectDuplicateImages -dCompressFonts=true -r150 -sOutputFile=suppl.pdf suppl_highRes.pdf

arxiv: full
	rm -rf ../arxiv.tar.gz ../paper_arXiv
	cd ../arxiv-latex-cleaner && python -m arxiv_latex_cleaner ../paper/
	# Unfortunately it still doesn't remove unused PDF etc files... need to use the arxiv-collector
	rm -f /tmp/latexmk
	cd .. && python arxiv-collector/arxiv_collector.py --get-latexmk /tmp/latexmk
	cd ../paper_arXiv && python ../arxiv-collector/arxiv_collector.py --latexmk /tmp/latexmk main.tex
	mv ../paper_arXiv/arxiv.tar.gz ../
	rm -rf ../paper_arXiv


